Diverse Rule Sets

While machine-learning models are flourishing and transforming many aspects of everyday life, the inability of humans to understand complex models poses difficulties for these models to be fully trusted and embraced. Thus, interpretability of models has been recognized as an equally important quality as their predictive power. In particular, rule-based systems are experiencing a renaissance owing to their intuitive if-then representation. However, simply being rule-based does not ensure interpretability. For example, overlapped rules spawn ambiguity and hinder interpretation. Here we propose a novel approach of inferring diverse rule sets, by optimizing small overlap among decision rules with a 2-approximation guarantee under the framework of Max-Sum diversification. We formulate the problem as maximizing a weighted sum of discriminative quality and diversity of a rule set. In order to overcome an exponential-size search space of association rules, we investigate several natural options for a small candidate set of high-quality rules, including frequent and accurate rules, and examine their hardness. Leveraging the special structure in our formulation, we then devise an efficient randomized algorithm, which samples rules that are highly discriminative and have small overlap. The proposed sampling algorithm analytically targets a distribution of rules that is tailored to our objective. We demonstrate the superior predictive power and interpretability of our model with a comprehensive empirical study against strong baselines.

==> deprecated.tex <==
\subsection{Others}

Advantages.
\begin{itemize}
    \item \cite{lakkaraju2016interpretable} does not have fine-grained level of control over the size of the decision set.
    \item Stronger approximation guarantees.
    \item Large coverage implicitly implies a shorter rule.
\end{itemize}

Potential improvements.
\begin{itemize}
    \item Include coverage of multi classes in quality.
    \item Use Partition Matroid to boudle a set of ``similar'' rules.
    \item Preprocessing to pre-mine accurate rules.
    \item Choose different $\nsel$, choose a turning point in the objective function.
    \item Two-level? As a partition matroid? Run the algorithm with a small $\nsel$ then followed by separate runs for each rule.
\end{itemize}


\subsection{Direct local pattern sampling}

A line of recent work devises an efficient two-step sampling procedure, which is capable of sampling from useful pattern distributions while obviates a burn-in period of Markov chains \cite{boley2011direct,boley2012linear}.
This technique first samples a data record and then samples an element from the powerset of the record.
The epitome of possible pattern distributions is the distribution proportional to pattern frequency, where each record $\tran$ is sampled with a probability proportional to $2^{|\tran|}$ and the element of the powerset of the record is sampled u.a.r.
The technique can extend the sampling space of data records to Cartesian product of records. %, and uniform sampling of powerset to a sampling proportional to cardinality of itemsets.
\cite{boley2012linear} further propose a framework for possible pattern distributions, which has a form
\eq{\distn(\itemset) \sim \fitem_\star(\itemset) \prod_{i} \fsupp(\dat_i(\itemset)), }
where $\star\in\{\prod, \sum\}$, $\fitem: \items \to \mathbb{R}_+$, $\fitem_\star(\itemset): \star_{i\in\itemset} \fitem(i)$ and $\fsupp\in\{\text{supp}, \bar{\text{supp}} \}$.

Despite its efficiency, there are some restrictions on the proposed discriminative pattern distribution.
\eq{\distn(\itemset) \sim \datplus(\itemset) (|\datminus| - \datminus(\itemset)).}
In imbalanced datasets, the distribution may be dominated by $|\datminus|$, and accurate and inaccurate itemsets with similar $\datplus(\itemset)$ are treated almost equally.
Furthermore, forcing the distribution to concentrate on mainly accurate itemsets requires high order Cartesian product, which is computationally heavy.


\subsection{A random walk for sampling accurate rules}
The simplest random walk is a walk over the itemset lattice by choosing a neighbor of the current itemset u.a.r., which converges to a stationary distribution proportional to the degree of an itemset.
Since every itemset has a constant degree, the stationary distribution is uniform.
By dropping all inaccurate itemsets, we obtain a random walk for accurate itemsets.
Unlike the work of \cite{boley2008randomized}, where they develop a random walk for frequent itemsets that never jumps into infrequent itemsets, the random walk for accurate itemsets has to go through inaccurate itemsets in order to reach all possible accurate itemsets. Otherwise the underlying graph may be disconnected.
Besides, it is trivial to find the most frequent itemset, i.e., the null itemset, whereas it is \np-hard to find the first accurate itemset.
\begin{figure} % default is [tbp], htbp.
\centering
\includegraphics[width=.35\textwidth]{pic/disconnected_accuracy.jpg} % options: width, height, totalheight, scale, angle
\caption{Disconnected accurate itemsets. Each oval represents an inaccurate singleton itemset.} \label{fig:disconnected_accuracy}
\end{figure}
\note[Guangyi]{An important difference b/w r.w. over itemsets and subgraphs is that every itemset has a constant degree.}
\note[Guangyi]{It seems that this r.w. has no advantage over a naive Monte Carlo method, sampling $2^{\items}$ u.a.r and checking accuracy?}

A natural extension is a random walk that converges to a distribution proportional to accuracy.
This can be achieved by Metropolis-Hastings algorithm \cite{al2009output}.
An example of such a random walk being slow in convergence can be constructed in a similar way as that in \cite{boley2008randomized}.
\begin{proposition}
The proposed random walk that converges to a distribution proportional to accuracy is not guaranteed to converge in polynomial time.
\end{proposition}
\begin{proof}
A counterexample can be constructed in a similar way as that in \cite{boley2008randomized}, where we are given three positive data records $\dat=\{ \{1\}, \{2,...,\ndat\}, \{\ndat+2,...,2\ndat\} \}$.
Any itemset that has a non-zero support is an exact accurate itemset, or otherwise a zero-accurate itemset.
The random will never visit zero-support itemsets since their acceptance ratio is zero. Therefore edges between an accurate itemset and an zero-accurate one degenerates into a self-loop.
We bound the mixing time via conductance. 
It is well-known that $\mixing(\epsilon) \ge \frac{1}{4\Phi} \log \frac{1}{2\epsilon}$.
Let $\setofitemset = \{1\} \cup \powerset(\{2,...,\ndat\}) \setminus \emptyset$.
\eq{
\Phi \le \Phi(\setofitemset) = \frac{\phi(\setofitemset)}{\distn(\setofitemset)} = 2\phi(\setofitemset) &= 2 \sum_{i=1}^\ndat \distn(\{i\}) \transmat(\{i\}, \emptyset)\\
&=2 \ndat \frac{1}{2^\ndat} \frac{1}{2(2\ndat)} = \frac{1}{2^{\ndat+1}}
}
\end{proof}

Hence, the major issue is potential slow convergence of the random walk. 
Besides, a guaranteed polynomial-time converged random walk for u.a.r. sampling should not be expected because of the hardness result.
\note[Guangyi]{Another pitfall of MCMC is the support information of the current itemset or neighboring itemsets need computing at every step, i.e., on-the-fly Markov chains.}


\subsection{Rejection sampling for direct local pattern sampling}
We propose a more efficient direct local pattern sampling method.
We start with a simple case where we sample an itemset with respect to a distribution proportional to its frequency.

\begin{theorem}
The proposed sampling method samples an itemset from a distribution proportional to its frequency.
\end{theorem}
\begin{proof}
First we sample \nsamptran records $\{\tran_i\}$ u.a.r. to estimate the partition function $\pttn=\sum_{\tran\in\trans} 2^{|\tran|}$.
\begin{align}
\tilde{\pttn} = \frac{|\trans|}{t} \sum_{i\in[t]} 2^{|\tran_i|}
\end{align}
Then we sample a record \tran with respect to probability $2^{|\tran|}/\tilde{\pttn}$ using rejection sampling.
I.e., we first sample a record \tran u.a.r., and then accept it with a probability $\frac{|\trans| 2^{|\tran|}}{\tilde{\pttn} \bigC}$ where \bigC is a large constant.
We repeat until we accept one record.
At the end we sample an itemset \itemset from $\powerset(\tran)$ u.a.r.
\begin{align}
P(\itemset) = \frac{\dat(\itemset)}{|\powerset(\tran)|} * 2^{|\tran|}/\tilde{\pttn} \propto \dat(\itemset)
\end{align}
The above equation holds in a sense of expectation.
\note[Guangyi]{$\tilde{\pttn}$ doesn't seem necessary? How is its variance of this estimator?}
\end{proof}

We can follow a similar scheme to sample discriminative itemsets,
where we instead sample a pair of records $(\tranplus,\tranminus)$ for partition function estimation and rejection sampling, with an acceptance ratio $\frac{|\datplus||\datminus| (2^{|\tranplus\setminus\tranminus|}-1) 2^{|\tranplus\cap\tranminus|}}{\tilde{\pttn} \bigC}$.


\subsection{First diversification formulation}
Our objective is to maximizing the following diversification function under a cardinality constraint $|\sel|\le\nsel$.
\eq{
\distq(\sel) = \quality(\sel) + \lambdaq\dist(\sel), \label{eq:obj}
}
where $\quality(\cdot)$ stands for a measure of monotone submodular quality, $\dist(\cdot)$ a measure of diversity, and $\lambdaq$ a user-defined hyperparameter to control the trade-off between previous two measures.
We now specify quality and diversity for a decision set in details.
Quality refers to a cover of correctly classified data points by $\sel$.
\eq{
\quality(\sel) = \sum_{\datelem\in\dat} \findicator(\exists \elem\in\sel \st \datelem\in\datplus(\elem)),
}
where $\datplus(\elem)=\{\datelem\in\dat | \elem(\datelem)=1, \lbl=1\}$.
Diversity refers to the sum of pairwise distances of elements in $\sel$, where a distance between two rules is defined to be the Jaccard distance of their covers over data points, which is a metric.
Note that maximizing the defined distance captures exactly the notion of small overlap.
\eq{
\dist(\sel) &= \sum_{\elem_i,\elem_j\in\sel} \dist(\elem_i,\elem_j)\\
\dist(\elem_i,\elem_j) &= 1 - \frac{|\dat(\elem_i) \cap \dat(\elem_j)|}{|\dat(\elem_i) \cup \dat(\elem_j)|},
}
where $\dat(\elem)=\{(\datelem,\lbl)\in\dat | \elem(\datelem)=1\}$.

Maximizing this new formulation will give a desirable decision set in terms of our goal.
Though $\dist(\cdot)$ may potentially favor rules with a small cover since they are less likely to overlap, $\quality(\cdot)$ eliminates this problem by encouraging a large cover.
On the contrary, while $\quality(\cdot)$ may give a high score to an inaccurate rule with a large cover, $\dist(\cdot)$ will counteract the inclusion of such rules due to their large coverage of incorrectly classified data points.
Therefore this two measures collaborate to produce a decision set that is both accurate and diverse.
\note[Guangyi]{Greedy algorithm will not work well here. $\dist(\cdot)$ is supermodular and thus the penalty for rules with a large cover grows as $|\sel|$ increases. In greedy, first selected rule will not be punished and may induce low accuracy.}


\subsection{Mine without pre-mining}

We obviate enumerating $\univ$ by replacing swapping in local search with a modification to one rule in current $\sel$.
We define a modification to be either adding or removing a feature into or from a rule.
A modification is \emph{good} if it increases the objective function.

Ways to cope with exponential size:
\begin{itemize}
	\item Ellipsoid methods
	\item Apriori
	\item DPP
	\item Column generation
	\item Graphical models
	\item Continuous relaxation\\
	Continuous greedy procedure; Linear SVM; Garg, p-term k-DNF rule weight vectors.
\end{itemize}
Tips:
\begin{itemize}
	\item Related work of Angelino.\\
	Can I prune significantly? Like branch-and-bound.
	\item Accuracy quality\\
	Proportional submodular?
	\item Try to formulate optim problem with features as decision vars. Any Ellipsoid or Col gen can be used?
\end{itemize}



\subsection{An attempt to directly transform \cite{lakkaraju2016interpretable} to diversification}

In the interpretable decision sets (\ids) proposed by \cite{lakkaraju2016interpretable}, they specify different desirable properties of a selected subset of decision rules.
Each property is formulated as a non-negative submodular function.
Thus the final objective function, a linear combination of properties, still enjoys (non-monotone) submodularity, which can be optimized effectively by forward-backward local search.

One key property among those proposed is small overlap of training data points, since large overlap between rules reduces interpretability.
This property is nasty to handle because it induces non-monotonity.
Thus the forward-backward local search is only able to give $3$-approximation.
However, if we adopt a new viewpoint, in which we consider the problem as selecting a set of diverse decision sets from a large collection, we are able to solve the same problem in $2$-approximation, thanks to all machinery brought from the field of diversity \cite{borodin2012max}.

Let us take a closer look at formulation of properties in \cite{lakkaraju2016interpretable}.
We have a set of labeled data points $\dat= \{ (\datelem_1,\lbl_1),...,(\datelem_\ndat,\lbl_\ndat) \}$.
We denote the universal set of rules as $\univ$ and the selected subset as $\sel$.
Simple modular properties include the cardinality of $\sel$, length of each rule in $\sel$, and size of misclassified data points of each rule in $\sel$.
\eq{
& \ppt_1(\sel) = |\univ| - |\sel| \\
& \ppt_2(\sel) = L_{\text{max}} \cdot |\univ| - \sum_{\elem\in\sel} \flength(\elem) \\
& \ppt_3(\sel) = |\dat| \cdot |\univ| - \sum_{\elem\in\sel} |\datminus(\elem)|
}
Submodular properties include the cover over labels and the cover over \dat.
\eq{
& \ppt_4(\sel) =  \sum_{\lbl\in\lbluniv} \findicator(\exists \elem\in\sel \st \flabel(\elem)=\lbl)\\
& \ppt_5(\sel) =  \sum_{\datelem\in\dat} \findicator(\exists \elem\in\sel \st \datelem\in\datplus(\elem))
}
The final property proposed by \cite{lakkaraju2016interpretable}, which is also the most important one in their paper, is small overlap.
\eq{
\ppt_6(\sel) = |\dat|\cdot|\univ|^2 - \sum_{\elem_i,\elem_j\in\sel} \foverlap(\elem_i,\elem_j)
}
\note[Guangyi]{Does $\ppt_3$ encourage small/long (specific) and accurate rules?}
Note that $\ppt_3$ may count each misclassified data point more than once, as a severe penalty for misclassification.

The problem of non-monotonicity is induced by negative modular properties in $\ppt_1,\ppt_2,\ppt_3$ and a negation of non-negative supermodular property in $\ppt_6$.
The main contribution of our paper is to transform the small overlap property $\ppt_6$ into \maxsum dispersion \cite{borodin2012max}.
Since small normalized overlap implicitly implies small cardinality of $\sel$, which also favors more general and thus shorter rules. Therefore $\ppt_1,\ppt_2$ can be safely dropped.
\note[Guangyi]{May normalized overlap, i.e., Jaccard distance induce undesirable consequences?}
$\ppt_4,\ppt_5$ are smoothly incorporated as monotone submodular quality in diversification framework.
The problem left is how to model accuracy of $\sel$.
\note[Guangyi]{Modeling big coverage and accuracy as quality at the same time seems hard. So we may simplify the problem to model accuracy as quality and sum of pairwise jaccard distances as dispersion.}
